RepQ: Generalizing Quantization-Aware Training for Re-Parametrized Architectures

Existing neural networks are memory-consuming and computationally intensive, making deploying them challenging in resource-constrained environments. However, there are various methods to improve their efficiency. Two such methods are quantization, a well-known approach for network compression, and re-parametrization, an emerging technique designed to improve model performance. Although both techniques have been studied individually, there has been limited research on their simultaneous application. To address this gap, we propose a novel approach called RepQ, which applies quantization to re-parametrized networks. Our method is based on the insight that the test stage weights of an arbitrary re-parametrized layer can be presented as a differentiable function of trainable parameters. We enable quantization-aware training by applying quantization on top of this function. RepQ generalizes well to various re-parametrized models and outperforms the baseline method LSQ quantization scheme in all experiments.

==> supp_acronyms.tex <==
\DeclareAcronym{nn}{
    short = NN,
    long = Neural Networks,
}

\DeclareAcronym{qat}{
    short = QAT,
    long = Quantization\-/Aware Training,
}

\DeclareAcronym{bn}{
    short = BN,
    long = Batch Normalization,
}

\DeclareAcronym{fp}{
    short = FP,
    long = Floating-Point
}

\DeclareAcronym{lr}{
    short = LR,
    long = Learning Rate
}

==> tables/ablation.tex <==
\begin{table}[H] 
\begin{center}
% \resizebox{\textwidth}{!}{% t H
\begin{tabular}{cccccc}
  \hline
  Precision & RepQ-BN & RepQ-Scaling & Merged & Merged+BN & RepQ-Scaling+BN \\ 
  \hline
  8 & \textbf{73.11} & 72.65 & 72.49 & 72.86   & TBD \\
  4 & \textbf{70.31} & 69.58 & 69.21 & 70.09   &  TBD\\
  \hline
\end{tabular}
\end{center}
% }
\caption{ImageNet top-1 accuracy for different Batch Normalization placements in RepVGG-A0.}
\label{table:ablation}
\end{table}

==> tables/edge.tex <==
\begin{table}[H]
    \centering
    \begin{tabular}{c c c c}
    \hline
         Model & BN & BNEst & \makecell{BN for 3x3, BNEst for 1x1} \\
         \hline
         RepVGG-A0 & 72.25 & 72.43 & \textbf{72.73} \\
         % \hline
         RepVGG-B0 & 75.25 & 75.38 & \textbf{75.42} \\
         \hline
    \end{tabular}
    \caption{Batch Normalization Estimation effect on RepVGG ImageNet accuracy.}
    \label{table:edge}
\end{table}
